A Survey on Autonomous Driving Datasets: Statistics, Annotation Quality, and a Future Outlook

Autonomous driving has rapidly developed and shown promising performance due to recent advances in hardware and deep learning techniques. High-quality datasets are fundamental for developing reliable autonomous driving algorithms. Previous dataset surveys either focused on a limited number or lacked detailed investigation of dataset characteristics. To this end, we present an exhaustive study of 265 autonomous driving datasets from multiple perspectives, including sensor modalities, data size, tasks, and contextual conditions. We introduce a novel metric to evaluate the impact of datasets, which can also be a guide for creating new datasets. Besides, we analyze the annotation processes, existing labeling tools, and the annotation quality of datasets, showing the importance of establishing a standard annotation pipeline. On the other hand, we thoroughly analyze the impact of geographical and adversarial environmental conditions on the performance of autonomous driving systems. Moreover, we exhibit the data distribution of several vital datasets and discuss their pros and cons accordingly. Finally, we discuss the current challenges and the development trend of the future autonomous driving datasets.

==> sections/s6_important_datasets_old.tex <==
\section{High-Influence Datasets}
\label{influence_impact}
This section describes the milestone autonomous driving datasets in the field of perception (\ref{perception_datasets}), prediction, planning, and control (\ref{prediction_planning_control_datasets}). We also exhibit datasets for end-to-end autonomous driving (\ref{e2e_datasets}).

\begin{figure*}
    \centering
    % \includesvg[width=\textwidth]{}
    \includegraphics[width=\textwidth]{figures/chronological_overview/chronological_overview_v4.pdf}
    \caption{Chronological overview. We show the top 50 datasets with the highest impact scores. This diagram records datasets from 2007 to 2023 (until the writing of this paper).}
    \label{fig:chronological_overview}
\end{figure*}

\input{tables_images/impact_score_p1}

\subsection{Perception Datasets}
\label{perception_datasets}
Perception datasets are critical for developing and optimizing autonomous driving systems. They enhance vehicle reliability and robustness by providing rich, multimodal sensory data, ensuring effective perception and understanding of surroundings.

We leverage the proposed dataset evaluation metrics (see \ref{evaluation_metrics}) to calculate the impact scores of the collected perception datasets, subsequently selecting the top 50 datasets based on these scores to create a chronological overview, shown in Fig.~\ref{fig:chronological_overview}. Concurrently, as described in \ref{sensing_domain_coperception_system}, we categorize datasets into onboard, V2X, drone, and others, choosing a subset from each to compile a comprehensive table of 50 datasets (Tab.~\ref{tab:50_datasets}). It is worth noting that the datasets in the table are sorted by impact score within their respective categories and do not represent the overall top 50. In the following part, we choose several datasets with the highest impact scores within each sensing source and exhibit them considering their published year.

\subsubsection{Onboard}
    \textbf{KITTI.} 
    KITTI~\cite{geiger2012we} has profoundly influenced the autonomous driving domain since its release in 2012. KITTI encompasses a variety of real-world driving scenarios recorded by various sensors, including cameras, LiDAR, and GPS/IMU. Its rich annotations and high-resolution sensor data have facilitated the development and benchmarking of numerous algorithms across a range of autonomous driving tasks, such as object detection, tracking, optical flow, depth estimation, and visual odometry.
    
    \textbf{Cityscapes.}
    Cityscapes~\cite{cordts2016cityscapes} comprises a vast collection of images captured explicitly in intricate urban environments. Through meticulous labeling, Cityscapes provides pixel-level segmentation for 30 different object classes, which include various vehicle types, pedestrians, roads, and traffic sign information. Given its complexity and richness, Cityscapes has become a standard benchmark for tasks such as semantic segmentation in urban scenarios.
    
    \textbf{SYNTHIA.}
    SYNTHIA~\cite{ros2016synthia} is a synthetic dataset in the realm of autonomous driving. The dataset includes 13,400 images with pixel-wise annotations for semantic segmentation. One of the standout attributes of SYNTHIA is its capability to bridge the gap between real-world and synthetic data, fostering the development of robust and transferable approaches across different domains. 
    
    \textbf{Virtual KITTI.}
    Virtual KITTI~\cite{gaidon2016virtual} crafts to closely mimic the original KITTI dataset through a virtual environment, distinguishing itself by delivering high-resolution video sequences encapsulating various traffic situations and environmental conditions. Similar to \cite{geiger2012we}, Virtual KITTI supports crucial autonomous driving tasks, including object detection, semantic segmentation, and object tracking.
    
    \textbf{VIPER.}
    VIPER~\cite{richter2017playing} is a synthetic dataset collected from driving, riding, and walking perspectives in a realistic virtual world, addressing the challenge of data scarcity and the high cost of labeling real-world data. VIPER contains over 250,000 video frames annotated with ground-truth data for low- and high-level vision tasks while encapsulating various weather conditions, lighting scenarios, and complex urban landscapes. Overall, VIPER presents a valuable and cost-effective tool for researchers to expedite the development of reliable and safe autonomous driving.
    
    \textbf{Apolloscapes.}
    Apolloscapes~\cite{huang2018apolloscape} offers more than 140,000 high-resolution frames with accurate bounding boxes and pixel-wise semantic labels, critical for training and validating autonomous vehicles' perception and navigation systems. Apolloscapes supports images and point clouds semantic segmentation, 2D/3D object detection, multi-object tracking, and lane segmentation, enabling the creation and evaluation of advanced and safe autonomous driving systems. 
    
    \textbf{SemanticKITTI.}
    SemanticKITTI~\cite{behley2019semantickitti} is a notable extension of the KITTI family, focusing on semantic segmentation in the autonomous driving field. SemanticKITTI consists of over 43,000 LiDAR point cloud frames, making it one of the largest datasets for 3D semantic segmentation in outdoor environments. SemanticKITTI provides precise labels for 28 categories, such as car, road, building, etc., achieving a robust benchmark for evaluating the performance of point cloud semantic segmentation methods, underpinning numerous studies and innovations in related domains.
    
    \textbf{nuScenes.}
    nuScenes~\cite{caesar2020nuscenes} stands as an essential contribution to the field of autonomous driving, offering a rich repository of data that addresses the diverse needs of perception systems. nuScenes leverages LiDAR, radars, and cameras to record data from different urban scenes from Boston and Singapore. It is worth mentioning that its six cameras provide a comprehensive perspective of the surrounding environment, making them widely utilized in multi-view object detection tasks. In conclusion, the nuScenes dataset is a cornerstone in developing autonomous driving technologies, supporting multi-tasks and applications, and setting new benchmarks in the field.
    
    \textbf{Waymo.}
    The Waymo Open Dataset~\cite{sun2020scalability}, introduced in 2019, significantly influences research and advancement in autonomous driving by providing an extensive size of multimodal sensory data with high-quality annotations. Key contributions of the Waymo dataset include its comprehensive coverage of driving conditions and geographics, which are pivotal for the robustness and generability of different tasks, such as detection, tracking, and segmentation.
    
    \textbf{BDD100K.}
    BDD100K~\cite{yu2020bdd100k} dataset, released by the Berkeley DeepDrive center in 2018, is a substantial and diverse driving dataset renowned for its size and diversity. It comprises 100,000 videos, each about 40 seconds in duration. Meanwhile, it offers various annotated labels for object detection, tracking, semantic segmentation, and lane detection. This extensive compilation of data prompts advancements in the autonomous driving community, establishing itself as a challenging and versatile platform for researchers and engineers to propose and refine algorithms.
    
    \textbf{RADIATE.}
    RADIATE~\cite{sheeny2021radiate} is the first public radar dataset, which contains 44,140 annotated frames gathered under several adversarial weather conditions, such as rain, fog, overcast, and snow. It also incorporates LiDAR and camera data, allowing full perception and understanding of the driving surroundings.
    
    \textbf{Argoverse~2.}
    As a sequel to Argoverse~1~\cite{chang2019argoverse}, Argoverse~2~\cite{wilson2023argoverse} introduces more diversified and complex driving scenarios, presenting the largest autonomous driving taxonomy to date. It captures various real-world driving scenarios across six cities and varying conditions. Argoverse~2 supports a wide range of essential tasks, including but not limited to 3D object detection, semantic segmentation, and tracking. In summary, the Argoverse 2 dataset offers numerous multimodal data of real-world driving scenarios, fostering innovations and advancements of algorithms and showing its substantial potential as a vital resource in autonomous driving.

\subsubsection{V2X}

    \textbf{V2VNet.}
    The dataset introduced by V2VNet~\cite{wang2020v2vnet} focuses on leveraging V2V communication to allow autonomous vehicles to share information and perceive the environment from multiple viewpoints, which is crucial for detecting occluded objects and predicting the behavior of other traffic participants. This dataset was created using a high-fidelity LiDAR simulator named Lidarsim~\cite{manivasagam2020lidarsim} that utilizes real-world data to generate realistic LiDAR point clouds for various traffic scenes. In conclusion, this work brings attention to the V2V as a promising avenue for improving the capabilities of autonomous vehicles.
    
    \textbf{DAIR-V2X.}
    DAIR-V2X~\cite{yu2022dair} is a pioneering resource in the Vehicle-Infrastructure Cooperative Autonomous Driving, providing large-scale, multi-modality, multi-view real-world data. The dataset is designed to tackle challenges such as the temporal asynchrony between vehicle and infrastructure sensors and the data transmission costs involved in such cooperative systems. The impact of the DAIR-V2X dataset on autonomous driving is significant because it sets a benchmark for complexities of vehicle-infrastructure cooperation thanks to its multiple scenarios from the real world.  
    
    \textbf{Rope3D.}
    Rope3D presented in \cite{ye2022rope3d} is an essential contribution to the perception systems, which addresses the critical gap in autonomous driving by leveraging data gathered from roadside cameras. Rope3D consists of 50,000 images under various environmental conditions, including different illumination (daytime, night, dusk) and weather scenarios (rainy, sunny, cloudy), ensuring a high diversity of data that reflects real-world complexities. Overall, the Rope3D dataset is a pioneering work that accelerates advancements in roadside perception for autonomous driving while being a critical tool for researchers and engineers to develop more robust and intelligent autonomous driving systems.
    
    \textbf{V2V4Real.}
    V2V4Real~\cite{xu2023v2v4real} is the first large-scale, real-world dataset to address V2V cooperative perception. The data was collected from two vehicles with multimodal sensors like LiDAR and cameras. V2V4Real focuses on a range of perception tasks, such as cooperation 3D object detection, cooperative 3D object tracking, and Sim2Real domain adaptation. This versatility makes it an invaluable resource for developing and benchmarking autonomous driving algorithms. 


\subsubsection{Drone}

    \textbf{UAVDT.}
    The UAVDT~\cite{du2018unmanned} dataset consists of 80,000 accurately annotated frames with up to 14 kinds of attributes, such as weather conditions, flying attitude, camera view, vehicle category, and occlusion levels. The dataset focuses on UAV-based object detection and tracking in urban environments. Moreover, the UAVDT benchmark includes high-density scenes with small objects and significant camera motion, all challenging for the current state-of-the-art methods.
    
    \textbf{DroneVehicle.}
    DroneVehicle~\cite{sun2022drone} proposes a large-scale drone-based dataset, which provides 28,439 RGB-Infrared image pairs to address object detection, especially under low-illumination conditions. Furthermore, it covers a variety of scenarios, such as urban roads, residential areas, and parking lots. This dataset is a significant step forward in developing autonomous driving technologies due to its unique drone perspective across a broad range of conditions.

\subsubsection{Others}

    \textbf{Pascal3D+.}
    Pasacal3D+~\cite{xiang2014beyond} is an extension of the PASCAL VOC 2022~\cite{everingham2010pascal},  overcoming the limitations of previous datasets by providing a richer and more varied set of annotations for images. Pasacal3D+ augments 12 rigid object categories, such as cars, buses, and bicycles, with 3D pose annotations and adds more images from ImageNet~\cite{deng2009imagenet}, resulting in a high degree of variability. 
    % It is important to exploit approaches that can perform well in diverse and unpredictable conditions in real driving conditions. 
    
    \textbf{TT 100K.}
    Tsinghua-Tencent 100K~\cite{zhu2016traffic} solves the challenges of detecting and classifying traffic signs in realistic driving conditions. It provides 100K images, including 30,000 traffic-sign instances. Beyond its large data size, the high-resolution images encompass a wide range of illumination and weather conditions, making it robust for training and validating traffic sign recognition.  
    
    \textbf{Mapillary Vistas.}
    Mapillary Vistas dataset, proposed by \cite{neuhold2017mapillary} in 2017, particularly aims at semantic segmentation of street scenes. The 25,000 images in the dataset are labeled with 66 object categories and include instance-specific annotations for 37 classes. It contains images from diverse weather, time of day, and geometric locations, which helps mitigate the bias towards specific regions or conditions.


\subsection{Prediction, Planning, and Control Datasets}
\label{prediction_planning_control_datasets}
Prediction, planning, and control datasets serve as the foundation for facilitating the training and evaluation of driving systems to forecast traffic dynamics, pedestrian movements, and other essential factors that influence driving decisions. By simulating myriad driving scenarios, they empower autonomous vehicles to make informed decisions, navigate complex environments, and maintain safety and efficiency on the road. Hence, we demonstrate in detail several high-impact datasets related to these tasks according to the data size, modalities, and citation number. We summarize the prediction, planning, and control datasets into task-specific and multi-task groups.
\input{tables_images/prediction_planning_control}
\subsubsection{Task-Specific Datasets}
    \textbf{highD.}
    The drone-based highD~\cite{krajewski2018highd} dataset provides a large-scale collection of naturalistic vehicle trajectories on German highways, containing post-processed trajectories of 110,000 cars and trucks. The dataset aims to overcome the limitations of existing measurement methods for scenario-based safety validation, which often fail to capture the naturalistic behavior of road users or to include all relevant data with sufficient quality. 
    
    \textbf{PIE.}
    The Pedestrian Intention Estimation (PIE) dataset proposed by \cite{rasouli2019pie} represents a significant advancement in understanding pedestrian behaviors in urban environments. It encompasses over 6 hours of driving footage recorded in downtown Toronto under various lighting conditions. The PIE dataset offers rich annotations for perception and visual reasoning, including bounding boxes with occlusion flags, crossing intention confidence, and text labels for pedestrian actions. The long continuous sequences and annotations facilitate multiple tasks like trajectory prediction and pedestrian intention prediction.
    
    \textbf{USyd.}
    USyd~\cite{zyner2019naturalistic} pushes the progress of the driver intention prediction in the context of urban intersections without traffic signals, which are common in urban settings and represent a challenge due to the lack of clear road rules and signals. The dataset incorporates over 23,000 vehicles traversing five different intersections, collected using a vehicle-mounted LiDAR-based tracking system. The data modalities included are exhaustive, providing vehicle tracks with lateral and longitudinal coordinates, heading, and velocity. This information is vital to predict driver behavior, accounting for the uncertainty inherent in human driving patterns.
    
    \textbf{Argoverse.}
    Argoverse~\cite{chang2019argoverse} is a crucial dataset in 3D object tracking and motion forecasting. Argoverse provides 360$^{\circ}$ images from 7 cameras, forward-facing stereo imagery, and LiDAR point clouds. The recorded data covers over 300K extracted vehicle trajectories from 290km of mapped lanes. With the assistance of rich sensor data and semantic maps, Argoverse is pivotal in advancing research and development in prediction systems.
    
    \textbf{inD.}
    The importance of the inD~\cite{bock2020ind} lies in its large-scale, high-quality, and diverse set of trajectory data crucial for several applications, including road user prediction models and scenarios-based safety validation for autonomous vehicles in urban intersection environments. It covers around 11,500 different road user trajectories, e.g., vehicles, bicyclists, and pedestrians. These trajectories have a positioning error of less than 0.1 meters, which is pivotal for the reliability of the data.
    
    \textbf{PePscenes.}
    PePscenes~\cite{rasouli2020pepscenes} tackles the requirement for understanding and anticipating pedestrian actions in dynamic driving surroundings. This dataset enhances the nuScenes~\cite{caesar2020nuscenes} dataset by adding per-frame 2D/3D bounding box and behavior annotations, focusing on pedestrian crossing actions. One of the key attributes of \cite{rasouli2020pepscenes} is incorporating various data types involving semantic maps, scene images, trajectories, and ego-vehicle states, which are necessary for creating robust models capable of understanding complex traffic scenarios.
    
    \textbf{openDD.}
    The openDD~\cite{breuer2020opendd} dataset focuses on analyzing and predicting traffic scenes around roundabouts, which are complex and unregulated by traffic lights. It is unique in leveraging drone-captured imagery with high resolution (4K), which spans over 62 hours of trajectory data from 501 separate flights. The dataset contains not only trajectories but also shapefiles and an extensible markup language (XML) file describing the road topology, along with a reference image for each underlying intersection.
    
    \textbf{nuPlan.}
    nuPlan~\cite{caesar2021nuplan} is the world's first closed-loop machine learning-based planning benchmark in autonomous driving. This multimodal dataset comprises around 1,500 hours of human driving data from four cities across America and Asia, featuring different traffic patterns, such as merges, lane changes, interactions with cyclists and pedestrians, and driving in construction zones. These characters of the nuPlan dataset take into account the dynamic and interactive nature of actual driving, allowing for a more realistic evaluation.
    
    \textbf{exiD.}
    The exiD~\cite{moers2022exid} trajectory dataset, presented in 2022, is a pivotal contribution to the highly interactive highway scenarios. It takes advantage of drones to record traffic without occlusion, minimizing the influence on traffic and ensuring high data quality and efficiency. This drone-based dataset surpasses previous datasets in terms of the diversity of interactions captured, especially those involving lane changes at highway entries and exits.
    
    \textbf{MONA.}
    The Munich Motion Dataset of Natural Driving (MONA)~\cite{gressenbuch2022mona} is an extensive dataset, with 702K trajectories from 130 hours of videos, covering urban roads with multiple lanes, an inner-city highway stretch, and their transitions. This dataset boasts an average overall position accuracy of 0.51 meters, which exhibits the quality of the data collected using highly accurate localization and LiDAR sensors.

\subsubsection{Multi-Task Datasets}

    \textbf{INTERACTION.}
    The INTERACTION~\cite{zhan2019interaction} dataset covers diverse, complex, and critical driving scenes, coupled with its comprehensive semantic map, allowing it to be a versatile platform for a multitude of tasks, such as motion prediction, imitation learning, and validation of decision and planning. Its inclusion of different countries further improves the robustness of analyzing the driving behavior across different cultures, which is critical for the global development of autonomous driving.
    
    \textbf{BLVD.}
    The BLVD~\cite{xue2019blvd} benchmark facilitates tasks such as dynamic 4D (3D+temporal) tracking, 5D (4D+interactive) interactive event recognition, and intention prediction, which are essential for a deeper understanding of traffic scenes. BLVD offers around 120K frames from different traffic scenes, comprising object density (low and high) and illumination conditions (daytime and nighttime). These frames are fully annotated with a large number of 3D labels incorporating vehicles, pedestrians, and riders. 
    
    \textbf{rounD.}
    The rounD dataset presented by \cite{krajewski2020round} is pivotal for scenario classification, road user behavior prediction, and driver modeling because of the large number of collections of road user trajectories at roundabouts. The dataset utilizes a drone equipped with a 4K resolution camera to collect over six hours of video, recording more than 13K road users. The broad recorded traffic situations and the high-quality recordings make rounD an essential dataset in autonomous driving, facilitating the study of naturalistic driving behaviors in public traffic.
    
    \textbf{Lyft Level 5.}
    Lyft Level 5~\cite{houston2021one} represents one of the most extensive autonomous driving datasets for motion prediction to date, with over 1,000 hours of data. It encompasses 17,000 25-second long scenes, a high-definition semantic map with over 15,000 human annotations, 8,500 lane segments, and a high-resolution aerial image of the area. It supports multiple tasks like motion forecasting, motion planning, and simulation. The numerous multimodal data with detailed annotations make the Lyft Level 5 dataset a vital benchmark for prediction and planning.
    
    \textbf{LOKI.}
    LOKI~\cite{girase2021loki}, standing for Long Term and Key Intentions, is an essential dataset in multi-agent trajectory prediction and intention prediction. LOKI tackles a crucial gap in intelligent and safety-critical systems by proposing large-scale, diverse data for heterogeneous traffic agents, including pedestrians and vehicles. This dataset makes a multidimensional view of traffic scenarios available by utilizing camera images with corresponding LiDAR point clouds, making it a highly flexible resource for the community.
    
    \textbf{SceNDD.}
    SceNDD~\cite{prabu2022scendd} introduces real driving scenarios that feature diverse trajectories and driving behaviors for developing efficient motion planning and path-following algorithms. It is also adaptable to different configurations of the ego-vehicle and contains a time horizon of prediction that can be broken down into timestamps for detailed analysis. In conclusion, the SceNDD dataset is a significant addition to autonomous driving prediction and planning research.
    
    \textbf{DeepAccident.}
    The synthetic dataset, DeepAccident~\cite{wang2023deepaccident}, is the first work that provides direct and explainable safety evaluation metrics for autonomous vehicles. The extensive dataset with 57K annotated frames and 285K annotated samples supports end-to-end motion and accident prediction, which is vital for improving the predictive capabilities of autonomous driving systems in avoiding collisions and ensuring safety. Moreover, this multimodal dataset is versatile for various V2X-based perception tasks, such as 3D object detection, tracking, and bird's-eye-view (BEV) semantic segmentation.
    
    \textbf{Talk2Bev.}
    The innovative dataset, Talk2BEV~\cite{dewangan2023talk2bev}, promotes the shift from traditional autonomous driving tasks to incorporate large vision-language models with BEV maps in the context of autonomous driving. Talk2BEV utilizes recent advances in vision-language models, allowing for a more flexible and comprehensive understanding of road scenarios. This dataset comprises over 20,000 diverse question categories, all human-annotated and derived from \cite{caesar2020nuscenes}. The proposed Talk2BEV-Bench benchmark can be leveraged across multiple tasks, covering decision-making, visual and spatial reasoning, and intent prediction.
    % This is critical to enable driving systems to interpret free-form natural language queries and ground these queries in a visual context, which is necessary for making informed decisions in real-time driving situations. 
    
    \textbf{V2X-Seq (Forecasting).}
    The trajectory forecasting dataset is a substantial part of the real-world dataset V2X-Seq~\cite{yu2023v2x}, containing about 80K infrastructure-view and 80K vehicle-view scenarios, and a further 50K cooperative-view scenarios. This diversity of sensing domains creates a more holistic view of the traffic environment, exhibiting huge potentiality for research and analysis on vehicle-infrastructure-cooperative (VIC) trajectory prediction. 


% Furthermore, several versatile datasets mainly focusing on perception, such as Waymo~\cite{sun2020scalability} and Argoverse~2~\cite{wilson2023argoverse}, also support tasks like motion prediction.

\subsection{End-to-End Datasets}
\label{e2e_datasets}
    End-to-end has become a growing trend as an alternative to modular-based architecture in autonomous driving~\cite{tampuu2020survey}. Several versatile datasets (like nuScenes~\cite{caesar2020nuscenes} and Waymo~\cite{sun2020scalability}) or simulators like CARLA~\cite{dosovitskiy2017carla} provide the opportunity to develop end-to-end autonomous driving. Meanwhile, some works present datasets that are especially for end-to-end driving.
    
    \textbf{DDD17.} The DDD17~\cite{binas2017ddd17} dataset is notable for its use of event-based cameras, which provide a concurrent stream of standard active pixel sensor (APS) images and dynamic vision sensors (DVS) temporal contrast events, offering a unique blend of visual data. Additionally, DDD17 captures diverse driving scenarios, including highway and city driving and various weather conditions, thus providing exhaustive and realistic data for training and testing end-to-end autonomous driving algorithms.

Other datasets summarized in this survey are shown in Tab.~\ref{all_dataset} Tab.~\ref{all_dataset2}, Tab.~\ref{all_dataset3}.
\input{tables_images/all_datasets}
\input{tables_images/all_datasets2}
\input{tables_images/all_datasets3}

% 
%     \textbf{highD.}
%     The drone-based highD~\cite{krajewski2018highd} dataset provides a large-scale collection of naturalistic vehicle trajectories on German highways, containing post-processed trajectories of 110,000 cars and trucks. The dataset aims to overcome the limitations of existing measurement methods for scenario-based safety validation, which often fail to capture the naturalistic behavior of road users or to include all relevant data with sufficient quality. 
%     \textbf{INTERACTION.}
%     The INTERACTION~\cite{zhan2019interaction} dataset covers diverse, complex, and critical driving scenes, coupled with its comprehensive semantic map, allowing it to be a versatile platform for a multitude of tasks, such as motion prediction, imitation learning, and validation of decision and planning. Its inclusion of different countries further improves the robustness of analyzing the driving behavior across different cultures, which is critical for the global development of autonomous driving.
%     \textbf{PIE.}
%     The Pedestrian Intention Estimation (PIE) dataset proposed by \cite{rasouli2019pie} represents a significant advancement in the understanding of pedestrian behaviors in urban environments. It encompasses over 6 hours of driving footage recorded in downtown Toronto under various lighting conditions. The PIE dataset offers rich annotations necessary for perception and visual reasoning, including bounding boxes with occlusion flags, crossing intention confidence, and text labels for pedestrian actions. The long continuous sequences and annotations facilitate multiple tasks like trajectory prediction and pedestrian intention prediction.
%     \textbf{BLVD.} \cite{xue2019blvd}
%     The BLVD~\cite{xue2019blvd} benchmark facilitates tasks such as dynamic 4D (3D+temporal) tracking, 5D (4D+interactive) interactive event recognition, and intention prediction, which are essential for a deeper understanding of traffic scenes. BLVD offers around 120K frames from different traffic scenes, comprising object density (low and high) and illumination conditions (daytime and nighttime). These frames are fully annotated with a large number of 3D labels incorporating vehicles, pedestrians, and riders. 
%     \textbf{USyd.}
%     USyd~\cite{zyner2019naturalistic} pushes the progress of the driver intention prediction in the context of urban intersections without traffic signals, which are common in urban settings and represent a challenge due to the lack of clear road rules and signals. The dataset incorporates over 23,000 vehicles traversing five different intersections, collected using a vehicle-mounted LiDAR-based tracking system. The data modalities included are exhaustive, providing vehicle tracks with lateral and longitudinal coordinates, heading, and velocity. This information is vital to predict driver behavior, accounting for the uncertainty inherent in human driving patterns.
%     \textbf{rounD.}
%     The rounD dataset presented by \cite{krajewski2020round} is pivotal for scenario classification, road user behavior prediction, and driver modeling because of the large number of collections of road user trajectories at roundabouts. The dataset utilizes a drone equipped with a 4K resolution camera to collect over six hours of video, recording more than 13K road users. The broad recorded traffic situations and its high-quality recordings make rounD an essential dataset in autonomous driving, facilitating the study of naturalistic driving behaviors in public traffic.
%     \textbf{inD.}
%     The importance of the inD~\cite{bock2020ind} lies in its large-scale, high-quality, and diverse set of trajectory data crucial for several applications, including road user prediction models and scenarios-based safety validation for autonomous vehicles in urban intersection environments. It covers around 11,500 different road user trajectories, e.g., vehicles, bicyclists, and pedestrians. These trajectories have a positioning error of less than 0.1 meters, which is pivotal for the reliability of the data.
%     \textbf{PePscenes.}
%     PePscenes~\cite{rasouli2020pepscenes} tackles the requirement for understanding and anticipating pedestrian actions in dynamic driving surroundings. The PePscenes dataset enhances the nuScenes~\cite{caesar2020nuscenes} dataset by adding per-frame 2D/3D bounding box and behavior annotations, focusing on pedestrian crossing actions. One of the key attributes of \cite{rasouli2020pepscenes} is incorporating various data types involving semantic maps, scene images, trajectories, and ego-vehicle states, which are necessary for creating robust models capable of understanding complex traffic scenarios.
%     \textbf{openDD.}
%     The openDD~\cite{breuer2020opendd} dataset focuses on analyzing and predicting traffic scenes around roundabouts, which are complex and unregulated by traffic lights. It is unique in leveraging drone-captured imagery with high resolution (4K), which spans over 62 hours of trajectory data from 501 separate flights. The dataset contains not only trajectories but also shapefiles and an extensible markup language (XML) file describing the road topology, along with a reference image for each underlying intersection.
%     \textbf{Lyft Level 5.}
%     Lyft Level 5~\cite{houston2021one} represents one of the largest autonomous driving datasets for motion prediction to date, with over 1000 hours of data. It encompasses 17,000 25-second long scenes, a high-definition semantic map with over 15,000 human annotations, 8,500 lane segments, and a high-resolution aerial image of the area. It supports multiple tasks like motion forecasting, motion planning, and simulation. The numerous multimodal data with detailed annotations make the Lyft Level 5 dataset serve as a vital benchmark for prediction and planning.
%     \textbf{LOKI.}
%     LOKI~\cite{girase2021loki}, standing for Long Term and Key Intentions, is an important dataset in the domain of multi-agent trajectory prediction and intention prediction. LOKI tackles a crucial gap in intelligent and safety-critical systems by proposing large-scale, diverse data for heterogeneous traffic agents, including pedestrians and vehicles. This dataset makes a multidimensional view of traffic scenarios available by utilizing camera images with corresponding LiDAR point clouds, making it a highly flexible resource for the community.
%     \textbf{nuPlan.}
%     nuPlan~\cite{caesar2021nuplan} is the world's first closed-loop machine learning-based planning benchmark in autonomous driving. This multimodal dataset comprises around 1500 hours of human driving data from four cities across America and Asia, featuring different traffic patterns, such as merges, lane changes, interactions with cyclists and pedestrians, and driving in construction zones. These characters of the nuPlan dataset take into account the dynamic and interactive nature of actual driving, allowing for a more realistic evaluation.
%     \textbf{exiD.}
%     The exiD~\cite{moers2022exid} trajectory dataset, presented in 2022, is a pivotal contribution to the highly interactive highway scenarios. It takes advantage of drones to record traffic without occlusion, minimizing the influence on traffic and ensuring high data quality and efficiency. This drone-based dataset surpasses previous datasets in terms of the diversity of interactions captured, especially those involving lane changes at highway entries and exits.
%     \textbf{MONA.}
%     The Munich Motion Dataset of Natural Driving (MONA)~\cite{gressenbuch2022mona} is an extensive dataset, with 702K trajectories from 130 hours of videos, covering urban roads with multiple lanes, an inner-city highway stretch, and their transitions. This dataset boasts an average overall position accuracy of 0.51 meters, which exhibits the quality of the data collected using highly accurate localization and LiDAR sensors.
%     \textbf{SceNDD.}
%     SceNDD~\cite{prabu2022scendd} introduces real driving scenarios that feature diverse trajectories and driving behaviors for developing efficient motion planning and path-following algorithms. It is also adaptable to different configurations of the ego-vehicle and contains a time horizon of prediction that can be broken down into timestamps for detailed analysis. In conclusion, the SceNDD dataset is a significant addition to autonomous driving prediction and planning research.
%     \textbf{DeepAccident.}
%     The synthetic dataset, DeepAccident~\cite{wang2023deepaccident}, is the first work that provides direct and explainable safety evaluation metrics for autonomous vehicles. The extensive dataset with 57K annotated frames and 285K annotated samples supports end-to-end motion and accident prediction, which is vital for improving the predictive capabilities of autonomous driving systems in avoiding collisions and ensuring safety. Moreover, this multimodal dataset is versatile for various V2X-based perception tasks, such as 3D object detection, tracking, and bird's eye view (BEV) semantic segmentation. 
% 


% \subsection{Planning}
% \label{planning_datasets}

% \subsection{Control}
% \label{control_datasets}
% introduce vlm control datasets like Talk2Car

==> tables_images/impact_score_p2.tex <==
\begin{table*}[!ht]
    \centering
    \setlength{\tabcolsep}{1.8pt}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{ccccccccccccccccccc}
        \toprule[1pt]
        \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Year}} & \multicolumn{1}{|c}{\multirow{2}{*}{\textbf{Size}}}  & \multirow{2}{*}{\textbf{Temp}} & \multicolumn{6}{c}{\textbf{Tasks number}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Categories}}} &\multirow{2}{*}{\textbf{Weather}} & \multirow{2}{*}{\textbf{Time of day}} & \multirow{2}{*}{\textbf{Scenraio type}} & \multirow{2}{*}{\textbf{Geometrical scope}} & \multirow{2}{*}{\textbf{Impact score}} \\
        ~ & ~ & \multicolumn{1}{|c}{~} & ~ & \textbf{2D Det} & \textbf{3D Det} & \textbf{2D Seg} & \textbf{3D Seg} & \textbf{Tracking} & \textbf{Lane Det} & \multicolumn{1}{c|}{~} & ~ & ~ & ~ & ~ & ~ \\
        \midrule[0.5pt]
        \multicolumn{16}{c}{Onboard} \\ 
        \midrule[0.5pt]
        nuScenes & 2020 & 40000 & 1 & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & 23 & 3 & 2 & 4 & 2 & 82.12 \\ 
        BDD100K & 2020 & 12000000 & 1 & - & - & - & - & - & - & 40 & 5 & 2 & 4 & 1 & 78.51 \\ 
        Waymo & 2020 & 230000 & 1 & - & - & - & - & - & - & 23 & 2 & 3 & 5 & 1 & 77.75 \\ 
        Cityscapes & 2016 & 25000 & 0 & - & - & - & - & - & - & 30 & 1 & 1 & 3 & 1 & 76.4 \\ 
        KITTI & 2012 & 41000 & 1 & - & - & - & - & - & - & 8 & 1 & 1 & 2 & - & 76.3 \\ 
        SYNTHIA & 2016 & 13400 & 0 & - & - & - & - & - & - & 13 & 2 & 3 & 5 & - & 69.44 \\ 
        Apolloscape & 2018 & 143906 & 1 & - & - & - & - & - & - & 28 & 4 & 3 & 3 & 1 & 67.97 \\ 
        Virtual KITTI & 2016 & 21260 & 1 & - & - & - & - & - & - & 8 & 3 & 2 & 5 & - & 66.61 \\ 
        SemanticKITTI & 2019 & 43552 & 1 & - & - & - & - & - & - & 28 & 1 & 1 & 4 & 1 & 65.66 \\ 
        PfBs & 2017 & 254064 & 1 & - & - & - & - & - & - & 11 & 4 & 3 & 4 & 1 & 65.27 \\ 
        PfD & 2016 & 24966 & 0 & - & - & - & - & - & - & 19 & 2 & 2 & 2 & - & 65.1 \\ 
        UA-Detrac & 2020 & 140000 & 1 & - & - & - & - & - & - & 4 & 3 & 4 & 2 & 1 & 63.8 \\ 
        Argoverse 2 & 2023 & 6000000 & 1 & - & - & - & - & - & - & 30 & 2 & 1 & 1 & 6 & 62.11 \\ 
        CityPerson & 2017 & 25000 & 0 & - & - & - & - & - & - & 30 & 2 & 1 & - & 27 & 61.85 \\ 
        Lane Det & 2017 & 133235 & 0 & - & - & - & - & - & - & 1 & 1 & 3 & 3 & 1 & 58.62 \\ 
        GTSDB & 2013 & 50900 & 0 & - & - & - & - & - & - & 4 & 2 & 2 & 3 & 1 & 58.39 \\ 
        CamVid & 2009 & 701 & 0 & - & - & - & - & - & - & 32 & 2 & 1 & 2 & 1 & 57.69 \\ 
        A2D2 & 2020 & 41277 & 0 & - & - & - & - & - & - & 38 & 2 & 1 & 3 & 3 & 57.26 \\ 
        IDD & 2019 & 10004 & 0 & - & - & - & - & - & - & 34 & 3 & 3 & 5 & 1 & 57.12 \\ 
        Foggy Cityscapes & 2018 & 20550 & 0 & - & - & - & - & - & - & 19 & 1 & 1 & 2 & 1 & 57.09 \\ 
        Caltech Ped & 2009 & 250000 & 0 & - & - & - & - & - & - & 1 & 1 & 1 & 1 & 2 & 56.64 \\ 
        Dr(eye)ve & 2018 & 555000 & 0 & - & - & - & - & - & - & 10 & 3 & 3 & 3 & - & 56.28 \\ 
        STF & 2020 & 13500 & 0 & - & - & - & - & - & - & 1 & 4 & 2 & 3 & 4 & 55.91 \\ 
        Virtual KITTI 2 & 2020 & 20992 & 1 & - & - & - & - & - & - & 8 & 4 & 2 & 3 & 1 & 55.74 \\ 
        RADIATE & 2021 & 44140 & 1 & - & - & - & - & - & - & 8 & 5 & 2 & 4 & 1 & 55.7 \\ 
        SHIFT & 2022 & 2500000 & 1 & - & - & - & - & - & - & 23 & 5 & 5 & 3 & - & 54.79 \\ 
        CAOS & 2022 & 13000 & 0 & - & - & - & - & - & - & 13 & 3 & 2 & 3 & - & 54.74 \\ 
        WoodScape & 2019 & 400000 & 0 & - & - & - & - & - & - & 40 & 1 & 1 & 3 & 3 & 53.98 \\ 
        KITTI-360 & 2021 & 150000 & 1 & - & - & - & - & - & - & 37 & 1 & 1 & 1 & 1 & 53.77 \\ 
        ACDC & 2021 & 4006 & 0 & - & - & - & - & - & - & 19 & 4 & 2 & 3 & 1 & 53.62 \\ 
        \midrule[0.5pt]
        \multicolumn{16}{c}{V2X} \\ 
        \midrule[0.5pt]
        % - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ \midrule[0.7pt]
        DAIR-V2X & 2022 & 71254 & 1 & - & - & - & - & - & - & 10 & 2 & 2 & 2 & 1 & 49.9 \\
        V2VNet & 2020 & 51200 & 1 & - & - & - & - & - & - & 1 & 1 & 1 & 1 & - & 43.94 \\ 
        V2XSet & 2022 & 11447 & 1 & - & - & - & - & - & - & 1 & 1 & 1 & 1 & - & 43.59 \\
        T\&J & 2019 & 100 & 1 & - & - & - & - & - & - & 1 & 1 & 1 & 2 & 1 & 42.78 \\ 
        Rope3D & 2022 & 50000 & 0 & - & - & - & - & - & - & 12 & 2 & 3 & 2 & 1 & 42.39 \\ 
        V2X-Sim & 2022 & 10000 & 1 & - & - & - & - & - & - & 23 & 1 & 1 & 1 & - & 40 \\ 
        A9-Dataset & 2022 & 1098 & 1 & - & - & - & - & - & - & 9 & 4 & 2 & 1 & 1 & 39.72 \\ 
        V2V4Real & 2023 & 40000 & 1 & - & - & - & - & - & - & 5 & 2 & 1 & 2 & 1 & 38.48 \\ 
        LUMPI & 2022 & 200000 & 1 & - & - & - & - & - & - & 3 & 6 & 3 & 1 & 1 & 34.87 \\ 
        AUTOCASTSIM & 2022 & 52000 & 1 & - & - & - & - & - & - & 1 & 1 & 1 & 1 & - & 34.49 \\ 
        \midrule[0.5pt]
        \multicolumn{16}{c}{Drone} \\ 
        \midrule[0.5pt]
        % - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ \midrule[0.7pt]
        UA-Detrac & 2020 & 140000 & 1 & - & - & - & - & - & - & 4 & 3 & 4 & 2 & 1 & 63.8 \\ 
        DroneVehicle & 2021 & 56878 & 0 & - & - & - & - & - & - & 5 & 1 & 3 & 4 & 1 & 43.89 \\ 
        Cooperative & 2020 & 10000 & 0 & - & - & - & - & - & - & 1 & 1 & 1 & 1 & - & 38.26 \\ 
        Stanford Aerial Ped & 2016 & 19000 & 0 & - & - & - & - & - & - & 6 & 1 & 1 & 1 & 1 & 27.07 \\ 
        \midrule[0.5pt]
        \multicolumn{16}{c}{Others} \\ 
        \midrule[0.5pt]
        % - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ \midrule[0.7pt]
        Mapillary Vistas  & 2017 & 25000 & 0 & - & - & - & - & - & - & 66 & 5 & 3 & 3 & 2 & 68.63 \\ 
        TT 100K & 2016 & 100000 & 0 & - & - & - & - & - & - & 45 & 2 & 2 & 2 & 10 & 63.99 \\ 
        Pascal3D+ & 2014 & 30899 & 0 & - & - & - & - & - & - & 12 & 2 & 2 & 1 & - & 57.87 \\ 
        WildDash & 2018 & 1800 & 0 & - & - & - & - & - & - & 28 & 2 & 2 & 7 & 1 & 49.02 \\ 
        TorontoCity & 2016 & 56000 & 0 & - & - & - & - & - & - & 4 & 2 & 2 & 1 & 1 & 44.82 \\ 
        DAWN & 2020 & 4543 & 0 & - & - & - & - & - & - & 5 & 6 & 3 & 3 & - & 42.99 \\   
        \bottomrule[1pt]
    \end{tabular}
    }
    \caption{Top 50 datasets}
\end{table*}
